Model Interpretability through the Lens of Computational Complexity

In spite of several claims stating that some models are more interpretable than others -- e.g., "linear models are more interpretable than deep neural networks" -- we still lack a principled notion of interpretability to formally compare among different classes of models. We make a step towards such a notion by studying whether folklore interpretability claims have a correlate in terms of computational complexity theory. We focus on local post-hoc explainability queries that, intuitively, attempt to answer why individual inputs are classified in a certain way by a given model. In a nutshell, we say that a class $\mathcal{C}_1$ of models is more interpretable than another class $\mathcal{C}_2$, if the computational complexity of answering post-hoc queries for models in $\mathcal{C}_2$ is higher than for those in $\mathcal{C}_1$. We prove that this notion provides a good theoretical counterpart to current beliefs on the interpretability of models; in particular, we show that under our definition and assuming standard complexity-theoretical assumptions (such as P$\neq$NP), both linear and tree-based models are strictly more interpretable than neural networks. Our complexity analysis, however, does not provide a clear-cut difference between linear and tree-based models, as we obtain different results depending on the particular post-hoc explanations considered. Finally, by applying a finer complexity analysis based on parameterized complexity, we are able to prove a theoretical result suggesting that shallow neural networks are more interpretable than deeper ones.

==> figures/perceptron.tex <==
%Note: I changed the format because according to the preliminaries the input is a row vector and the weights is a colomns vector.
$\begin{pmatrix} x_{\text{OrigCont}}, \, x_{\text{WellMotiv}}, \, x_{\text{FullTypos}}, \, x_{\text{EstAuthors}}\end{pmatrix}
\cdot
\begin{pmatrix} 2 \\ 1.3 \\ -0.5 \\ 0.6 \end{pmatrix}   \, -2.1 \geq \, 0$

%$\begin{pmatrix} 2, \, 1.3,\,-0.5,\,0.6 \end{pmatrix} \cdot \begin{pmatrix} 
%x_{\text{OrigCont}} \\ x_{\text{WellMotiv}} \\ x_{\text{FullTypos}} \\ x_{\text{EstAuthors}}\end{pmatrix} \, \geq \, 2.1$
%$2\times x_{\text{OriginalContent}} + 1.3\times x_{\text{WellMotivated}}\\
%- .5\times x_{\text{FullOfTypos}} + .6\times x_{\text{EstablishedAuthors}}\\ \geq 2.1
%$

